Towards General Visual-Linguistic Face Forgery Detection(V2)

Face manipulation techniques have achieved significant advances, presenting serious challenges to security and social trust. Recent works demonstrate that leveraging multimodal models can enhance the generalization and interpretability of face forgery detection. However, existing annotation approaches, whether through human labeling or direct Multimodal Large Language Model (MLLM) generation, often suffer from hallucination issues, leading to inaccurate text descriptions, especially for high-quality forgeries. To address this, we propose Face Forgery Text Generator (FFTG), a novel annotation pipeline that generates accurate text descriptions by leveraging forgery masks for initial region and type identification, followed by a comprehensive prompting strategy to guide MLLMs in reducing hallucination. We validate our approach through fine-tuning both CLIP with a three-branch training framework combining unimodal and multimodal objectives, and MLLMs with our structured annotations. Experimental results demonstrate that our method not only achieves more accurate annotations with higher region identification accuracy, but also leads to improvements in model performance across various forgery detection benchmarks. Our Codes are available in https://github.com/skJack/VLFFD.git.

==> sec/3_method.tex <==

\begin{figure*}[!t]
    \begin{center}
    
       \includegraphics[width=1.0\linewidth]{figures/main.pdf}
    \end{center}
       \caption{ Overall framework of the Prompt Forgery Image Generator (PFIG). The paired forgery and real image are first fed into the Mask Generation module to generate forgery mask $M$. Then the Forgery Region Extraction module extracts the selected region $R_s$. Subsequently, the Forgery Type Decision module and Forgery Blending module decide the fine-grained forgery types of $R_s$ and generate the mixed forgery image, respectively.
       Finally, the fine-grained prompt is generated by the forgery region and types with the template.
       }
    \label{fig:pfig}
\end{figure*}
\begin{figure}[!t]
    \begin{center}
    
       \includegraphics[width=1\linewidth]{figures/type_1.pdf}
    \end{center}
       \caption{Five typical types of forgery faces. (a) Color Difference. (b) Blur. (c) Structure Abnormal.
       (d) Texture Abnormal. (e) Blend Boundary.
       The red circle highlights the region of each forgery type. (Best viewed in color.)
       }
    \label{fig:type}
\end{figure}

\section{Face Forgery Text Generator}

In this section, we introduce our proposed FFTG pipeline, which comprises the Raw Annotation Generation and Annotation Refinement with mllm. 
\subsection{Raw Annotation Generation}

PFIG aims to generate mixed forgery images with fine-grained annotations from an existing paired face forgery dataset. It disentangles forgery traces in the dataset into \textbf{regions} and \textbf{types}--- two key elements of forgeries~\cite{chen2022self,shiohara2022detecting}. As illustrated in Fig.~\ref{fig:pfig}, given a real image $i_r \in \mathbb{R}^{ 3\times H \times W}$ and its corresponding forgery image $i_f \in \mathbb{R}^{ 3\times H \times W}$, PFIG encompasses the following steps:


    \textbf{Mask Generation}. To locate the forgery region, similar to~\cite{chen2021local}, we first construct manipulated mask $M$ by computing the absolute pixel-wise difference in the RGB channels, and then normalizing it to the range of $[0,1]$:
    \begin{equation}
        M = |i_r-i_f| / 255.
        \label{equation:1}
    \end{equation}
    
    % \item 
    \textbf{Forgery Region Extraction}. 
    % This step aims to choose one forgery region that contains the $i_f$.
    % Specially, we divide the facial image into four regions based on landmarks, including mouth, nose, eyes, and face. 
    % Then, we calculate the average value of $M$ within each region area, and empirically determine the threshold $\theta$ to obtain the forgery regions list $L_f$. That is:
    % \begin{equation}
    %     \frac{1}{|R_t|}\sum_{j\in R_t}M(j) > \theta, R_t \rightarrow L_f,
    %     \label{equation:2}
    % \end{equation}
    % where $R_t$ is one of the regional areas of the predefined four regions, $|R_t|$ represented the sum of pixels within the region $t$. If the value is greater than the $\theta$, the corresponding region is appended into regions list $L_f$.
    % After looping the Eq.~\ref{equation:2} with four regions, we randomly select one region $R_s$ from $L_f$ for the next step. The $R_s(i_r)$ and $R_s(i_f)$ represent the forgery region of the real and fake pixels, respectively.
    This step aims to select a forgery region containing $i_f$. Facial images are divided into four areas: mouth, nose, eyes, and face, based on landmarks. We compute the average value of $M$ in each area and set a threshold $\theta$ to form the forgery region list $L_f$. This is defined as:
    \begin{equation}
        \frac{1}{|R_t|}\sum_{j\in R_t}M(j) > \theta, R_t \rightarrow L_f,
        \label{equation:2}
    \end{equation}
    where $R_t$ represents one of the four predefined areas, and $|R_t|$ is the sum of pixels in area $t$. If the value exceeds $\theta$, the corresponding area is included in $L_f$. After processing all four areas, we randomly select one region $R_s$ from $L_f$ for the next step. $R_s(i_r)$ and $R_s(i_f)$ represent the forgery regions for real and fake pixels, respectively.
    
    \textbf{Forgery Type Decision}. The goal of this step is to determine the type of forgery via a specially designed criterion.
    According to the previous work and our observation, we categorize the existing forgery types as color difference, blur, structure abnormal, texture abnormal, and blend boundary as shown in Fig~\ref{fig:type}. We detail each forgery type and corresponding evaluation standard as follows:
    1) \textbf{Color Difference }: Occurs in face swaps with notable color variance. We assess this using the distance of average channel-wise mean and variance in $Lab$ color space between real and fake regions.
    2) \textbf{Blur}: We use the Laplacian operator to quantify local blurring in forgery faces, determining blurriness by the variance after applying the operator to real and fake images in the selected region.
    3) \textbf{Structure Abnormal}: Observed deformations in fake face organs are assessed using the SSIM index difference between real and fake images in the selected region $R_s$.
    4) \textbf{Texture Abnormal}: We measure texture clarity using the contrast of the Gray-Level Co-occurrence Matrix (GLCM), defining an area as texture abnormal when the real region's $C_d$ exceeds that of the fake beyond a threshold.
    5) \textbf{Blend Boundary}: Existing face manipulation methods
    conduct blending operation to transfer an altered face into an existing background, which leaves intrinsic cues across the blending boundaries~\cite{li2020face}, such as the red circle of Fig.~\ref{fig:type}(e). However, we find it difficult to directly detect the blend boundaries, especially if the forged image is of high quality. We thus enhance this trace by adjusting the blend methods and ratio in the next step.


    % \item  
    \textbf{Forgery Blending}.
    To diversify the mixed forgery image $i_m$, we utilize either Poisson or alpha blending based on a probability, formulated as:
    \begin{equation}
        \label{eq6}
        \left\{
        \begin{aligned}
            i_m =  & \alpha * R_s(i_f) + (1-\alpha)*i_r, &p<\theta_b\\
            i_m =  & Poisson(R_s(i_f),i_r),& p>\theta_b,
        \end{aligned}
        \right.
    \end{equation}
    Here, $\alpha$ controls the blending degree, $Poisson$ denotes standard Poisson blending, $p$ is a uniformly distributed random variable, and $\theta_b$ is a threshold dictating the probability of the two blending methods. Unlike Poisson blending that smoothens boundaries through gradient regularization, alpha blending creates distinct blending cues. Thus, we classify the forgery type as Blend Boundary when opting for alpha blending.




Supplementary materials provide detailed pseudocodes for each forgery type criterion. To integrate fine-grained annotations and adapt the pre-trained upstream model, we create sentence-level fine-grained prompts $P$ for each mixed forgery image using the template \textit{``this is a fake person, the forgery region is \_\_ , the forgery type is \_\_"} where the first blank is filled with the selected forgery region $R_s$, and the second with the corresponding forgery types. This differs from regular multimodal tasks requiring raw image descriptions, as recent studies show that CLIP can achieve SOTA performance with simple templated text. We adopt this approach by using a specially designed cloze format for our prompts to fine-tune CLIP, enhancing its ability to discern face regions and forgery types.

\subsection{Coarse-and-Fine Co-training Framework}
In this section, we introduce our learning framework adopted by the multimodal co-training mechanism. Specifically, the original data with coarse-grained prompts are trained by Coarse-grained Multimodal Learning (CML) to let $E_i$ and $E_t$ obtain the basic discrimination.
Meanwhile, Fine-grained Multimodal Learning (FML) further guides and refines the encoders to learn more generalized cues by learning from rich supervision semantic information. 
\begin{figure}[t]
    \begin{center}
       \includegraphics[width=1\linewidth]{figures/finetune.pdf}
    \end{center}
       \caption{Paradigm of our VLFFD. The traditional method trains a unimodal encoder via digitized binary labels and can only output the probability of real or fake during test time. Our method trained multimodal encoders
       with generated mixed forgery image and the fine-grained language-level annotation and can output the similarity score between the visual and sentence, which is more interpretable. Furthermore, the performance of our method outperforms the baseline $13\%$ under the unseen test data in terms of AUC.
       (Best viewed in color.)
       }
    \label{fig:intro}
\end{figure}

\noindent\textbf{Coarse-grained Multimodal Learning.}
To effectively adapt the multimodal learning framework, we first convert the digitized binary labels (0 for real and 1 for forgery) into prompts. It's a strategic adaptation to align with the pre-trained model CLIP, facilitating the activation of its inherent semantic knowledge. After trying several templates,
we choose \textit{``this is a fake person"} for the forgery image and \textit{``this is a real person"} for the real one as the coarse-grained language prompts. 
Then, the real and forgery prompts are fed into the text encoder $E_t$ and concentrated together to form a coarse-grained language feature, represented as $l_c \in R^{2 \times D}$. Given the input data $x \in R^{B\times 3 \times H \times W}$ (B is the batch size)
with label $y \in \{0,1\}$, the visual feature $v_c \in R^{B\times D} $ (D is the feature dimension) is obtained by the image encoder $E_i$. We use normalized cosine similarity as the metric of two modalities features denoted as $s(u,v) = \frac{u.v^T}{||u|||v||}$.
The coarse-grained loss $L_c$ based on cross-entropy loss can be defined as:
\begin{equation}
    L_{c} = -\frac{1}{B}\sum y log(s(v_c,l_c)).
\end{equation}


\noindent\textbf{Fine-grained Multimodal Learning.}  
To efficiently exploit the sentence-level knowledge, inspired by the visual-language pre-trained methods~\cite{radford2021learning}, we use the multimodal contrastive learning framework, which pulls the paired image and text representations close to each other.
Specifically, a batch of mixed forgery images $x_f \in R^{N \times 3 \times H \times W}$ ($N$ is the batch size) with prompt $p_f \in P$, are fed into the image encoder $E_i$ and text encoder $E_t$ to extract visual and language features $v_f \in R^{B \times D}$ and $l_f\in R^{B \times D}$, respectively, where $D$ is the dimension of the feature. Then, we compute the symmetric normalized cosine similarities between two modalities 
$s(v_f,l_f)$ and $s(l_f,v_f) \in R^{B\times B}$. The diagonal elements of the two symmetric matrices represent the similarity of paired features, while others are mismatched. Thus, we define the symmetric cross-entropy loss as the fine-grained loss $L_{f}$, which maximizes the diagonal of the two similarity matrices as follows:
\begin{equation}
    L_{f} = -\frac{1}{2N}(\sum log(s(v_f,l_f) \odot I) + \sum log(s(l_f,v_f) \odot I)),
\end{equation}
where $I \in R^{N \times N}$ represents the identity matrix. Since the beginning of the fine-grained prompt is the forgery coarse prompt, the $L_f$ can not only 
help encoders extract discriminative representations but also encourage the image encoder to extract refined features that promote generalization.


% \noindent\textbf{Text Enhancement.}
% To further enhance language diversity, we have leveraged a large language model (LLM) to expand our template. This allows us to generate multiple alternative templates, thereby enriching our training data. Specifically, during the training process, we expanded our fine-grained annotation using the LLM and randomly replaced a chosen template for the original one with a probability $p$. This strategy not only increases linguistic variety but also taps into the latent semantic knowledge of the pre-trained model.



\noindent\textbf{Overall Loss Function.} Considering both the
coarse-grained loss and fine-grained loss, the overall loss for our proposed framework is:
\begin{equation}
    L = L_c + \phi L_f,
\end{equation}
where $\phi$ is the hyperparameter used to scale the fine-grained loss. 


==> table/ablation1.tex <==
% \begin{table*}[t]
%     \centering
%     \resizebox{\textwidth}{!}{
%     \begin{tabular}{c|c|c|c|c|c|c}
%         \hline
%         %\multicolumn{4}{|c|}{GCD-AVG}\\
%         %\hline
%         Common-AUG&Inter-contrastive&Data Views Generation& Hard sample &Intra-contrastive &Celeb-DF&DFD\\
%         \hline
%         \checkmark&&&&&68.52&87.37\\
%         \hline
%         \checkmark&&\checkmark&&&74.12&88.32\\
%         \hline
%         \checkmark&\checkmark&&&&76.81&88.03\\
%         \hline
%         \checkmark&\checkmark&\checkmark&&&79.34&89.24\\
%         \hline
%         \checkmark&\checkmark&&\checkmark&&78.84&89.89\\
%         \hline
%         \checkmark&\checkmark&\checkmark&\checkmark&&80.3&90.12\\
%         \hline
%         \checkmark&\checkmark&\checkmark&\checkmark&\checkmark&\textbf{82.30}&\textbf{91.66}\\
%         \hline
%     \end{tabular}
%     }
%     \vspace{-2pt}
%     \caption{}
%     \label{table:5}
% \end{table*}
% \begin{table}[!t]
%     \centering
%     \renewcommand\arraystretch{1.2}
%     \resizebox{\columnwidth}{!}{
%     \begin{tabular}{cccc|c|c}
%         \hline
%         %\multicolumn{4}{|c|}{GCD-AVG}\\
%         %\hline
%         Inter&Views& Hard & Intra &Celeb-DF&DFD\\
%         \hline
%         % &&&&68.52&87.37\\
%         &\checkmark&&&74.12&88.32\\
%         \hline
%         \checkmark&&&&76.81&88.03\\
%         \hline
%         \checkmark&\checkmark&&&79.34&89.24\\
%         \hline
%         \checkmark&&\checkmark&&78.84&89.89\\
%         \hline
%         \checkmark&\checkmark&\checkmark&&80.30&90.12\\
%         \hline
%         \checkmark&\checkmark&\checkmark&\checkmark&\textbf{82.30}&\textbf{91.66}\\
%         \hline
%     \end{tabular}
%     }
%     \vspace{-2pt}
%     \caption{Ablation study on the influence of 
%     different components. Specifically, ``Instance" means instance contrastive learning module, ``views" represents our special designed data views generation strategy, ``hard" indicate the hard sample generation, and ``self" is short for the self-contrastive learning module.}
%     \label{table:5}
% \end{table}

% \begin{table}[!h]
%     \centering
%     \renewcommand\arraystretch{1.2}
%     \resizebox{\columnwidth}{!}{
%     \begin{tabular}{c|cc|cc}
%         \hline
%         %\multicolumn{4}{|c|}{GCD-AVG}\\
%         %\hline
%         \multirow{2}*{Method} & \multicolumn{2}{c|}{Celeb-DF}&
%         \multicolumn{2}{c}{DFDC-P}  \\

%         \cline{2-5}
%         % \cmidrule{2-5}
%         & AUC& EER &AUC& EER \\
%         \hline
%         Unimodal+Coarse&77.62&29.34&76.31&31.06\\
%         Unimodal+Fine&77.71&29.31&79.30&24.83\\
%         Multimodal+Coarse&80.79&25.16&81.79&26.13\\
%         Multimodal+C2F&\textbf{84.80}&\textbf{22.73}&\textbf{84.74}&\textbf{23.43}\\
%         \hline
%     \end{tabular}
%     }
%     \vspace{-2pt}
%     \caption{Ablation study on the impact of language information in terms of AUC and EER. The Unimodal and Multimodal represents whether convert the digital label into prompt and whether use the text-encoder. Coarse and 
%     Fine means granularity of the label. C2F represents our Coarse-and-Fine Co-training framework.
%     }
%     \label{table:ab1}
% \end{table}
\begin{table}[!t]
    \centering
    \renewcommand\arraystretch{1.2}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{c|c|cc|cc}
        \hline
        %\multicolumn{4}{|c|}{GCD-AVG}\\
        %\hline
        \multirow{2}*{Language}&\multirow{2}*{PFIG} & \multicolumn{2}{c|}{Celeb-DF}&
        \multicolumn{2}{c}{DFDC-P}  \\

        \cline{3-6}
        % \cmidrule{2-5}
        && AUC& EER &AUC& EER \\
        \hline
        $\times$&$\times$&77.62&29.34&76.31&31.06\\
        $\times$&$\checkmark$&77.71&29.31&77.30&29.83\\
        $\checkmark$&$\times$&80.79&25.16&81.79&26.13\\
        $\checkmark$&$\checkmark$&\textbf{84.80}&\textbf{22.73}&\textbf{84.74}&\textbf{23.43}\\
        \hline
    \end{tabular}
    }
    \vspace{-2pt}
    \caption{Ablation study on the impact of different components in terms of AUC and EER. `Language' indicates the conversion of digital labels into text prompts. `PFIG' signifies the implementation of Fine-grained Multimodal Learning.
    }
    \label{table:ab1}
\end{table}


==> table/ablation2.tex <==
% \begin{table*}[t]
%     \centering
%     \resizebox{\textwidth}{!}{
%     \begin{tabular}{c|c|c|c|c|c|c}
%         \hline
%         %\multicolumn{4}{|c|}{GCD-AVG}\\
%         %\hline
%         Common-AUG&Inter-contrastive&Data Views Generation& Hard sample &Intra-contrastive &Celeb-DF&DFD\\
%         \hline
%         \checkmark&&&&&68.52&87.37\\
%         \hline
%         \checkmark&&\checkmark&&&74.12&88.32\\
%         \hline
%         \checkmark&\checkmark&&&&76.81&88.03\\
%         \hline
%         \checkmark&\checkmark&\checkmark&&&79.34&89.24\\
%         \hline
%         \checkmark&\checkmark&&\checkmark&&78.84&89.89\\
%         \hline
%         \checkmark&\checkmark&\checkmark&\checkmark&&80.3&90.12\\
%         \hline
%         \checkmark&\checkmark&\checkmark&\checkmark&\checkmark&\textbf{82.30}&\textbf{91.66}\\
%         \hline
%     \end{tabular}
%     }
%     \vspace{-2pt}
%     \caption{}
%     \label{table:5}
% \end{table*}
% \begin{table}[!t]
%     \centering
%     \renewcommand\arraystretch{1.2}
%     \resizebox{\columnwidth}{!}{
%     \begin{tabular}{cccc|c|c}
%         \hline
%         %\multicolumn{4}{|c|}{GCD-AVG}\\
%         %\hline
%         Inter&Views& Hard & Intra &Celeb-DF&DFD\\
%         \hline
%         % &&&&68.52&87.37\\
%         &\checkmark&&&74.12&88.32\\
%         \hline
%         \checkmark&&&&76.81&88.03\\
%         \hline
%         \checkmark&\checkmark&&&79.34&89.24\\
%         \hline
%         \checkmark&&\checkmark&&78.84&89.89\\
%         \hline
%         \checkmark&\checkmark&\checkmark&&80.30&90.12\\
%         \hline
%         \checkmark&\checkmark&\checkmark&\checkmark&\textbf{82.30}&\textbf{91.66}\\
%         \hline
%     \end{tabular}
%     }
%     \vspace{-2pt}
%     \caption{Ablation study on the influence of 
%     different components. Specifically, ``Instance" means instance contrastive learning module, ``views" represents our special designed data views generation strategy, ``hard" indicate the hard sample generation, and ``self" is short for the self-contrastive learning module.}
%     \label{table:5}
% \end{table}
% \begin{table}[!h]
%     \centering
%     \renewcommand\arraystretch{1.2}
%     \resizebox{\columnwidth}{!}{
%     \begin{tabular}{c|c|cc|cc}
%         \hline
%         %\multicolumn{4}{|c|}{GCD-AVG}\\
%         %\hline
%         &\multirow{2}*{Backbone} & \multicolumn{2}{c|}{WDF}&
%         \multicolumn{2}{c}{DFDC-P}  \\

%         \cline{3-6}
%         % \cmidrule{2-5}

%         && AUC& EER &AUC& EER \\
%         \hline
%         \multirow{4}*{CNN}&Xception(IN)&66.17&40.14&69.80&35.41\\
%         &Xception(IN)+Ours&\textbf{70.22}&\textbf{37.37}&\textbf{76.11}&\textbf{30.65}\\
%         \cline{2-6}

%         &EN-B4(IN)&61.04&45.34&70.12&34.54\\
%         &EN-B4(IN)+Ours&\textbf{71.35}&\textbf{36.22}&\textbf{78.32}&\textbf{29.03}\\
%         \hline
%         \multirow{4}*{Transformer}&ViT-B(IN)&65.39&38.11&68.03&36.06\\
%         &ViT-B(IN)+Ours&74.64&30.94&75.31&30.69\\
%         &ViT-B(CLIP)+Ours&\textbf{78.80}&\textbf{27.81}&\textbf{78.00}&\textbf{29.60}\\
%         \cline{2-6}
%         &ViT-L(IN)&69.92&36.20&71.33&33.76\\
%         &ViT-L(IN)+Ours&76.49&30.49&79.53&79.53\\
%         &ViT-L(CLIP)+Ours&\textbf{84.80}&\textbf{22.73}&\textbf{84.74}&\textbf{23.43}\\
%         \hline
%     \end{tabular}
%     }
%     \vspace{-2pt}
%     \caption{Ablation study on the influence of 
%     different components. Specifically, ``Instance" means instance contrastive learning module, ``views" represents our special designed data views generation strategy, ``hard" indicate the hard sample generation, and ``self" is short for the self-contrastive learning module.}
%     \label{table:ab2}
% \end{table}

\begin{table}[!t]
    \centering
    \renewcommand\arraystretch{1.2}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{c|c|c|cc|cc}
        \hline
        %\multicolumn{4}{|c|}{GCD-AVG}\\
        %\hline
        \multirow{2}*{Backbone}&\multirow{2}*{CLIP}&\multirow{2}*{VLFFD} & \multicolumn{2}{c|}{WDF}&
        \multicolumn{2}{c}{DFDC-P}  \\

        \cline{4-7}
        % \cmidrule{2-5}

        &&& AUC& EER &AUC& EER \\
        \hline
        \multirow{2}*{Xception}&$\times$&$\times$&66.17&40.14&69.80&35.41\\
        &$\times$&$\checkmark$&\textbf{70.22}&\textbf{37.37}&\textbf{76.11}&\textbf{30.65}\\
        \cline{1-7}

        \multirow{2}*{EN-B4}&$\times$&$\times$&61.04&45.34&70.12&34.54\\
        &$\times$&$\checkmark$&\textbf{71.35}&\textbf{36.22}&\textbf{78.32}&\textbf{29.03}\\
        \hline
        \multirow{3}*{ViT-B}&$\times$&$\times$&65.39&38.11&68.03&36.06\\
        &$\times$&$\checkmark$&74.64&30.94&75.31&30.69\\
        &$\checkmark$&$\checkmark$&\textbf{78.80}&\textbf{27.81}&\textbf{78.00}&\textbf{29.60}\\
        \cline{1-7}
        \multirow{3}*{ViT-L}&$\times$&$\times$&69.92&36.20&71.33&33.76\\
        &$\times$&$\checkmark$&76.49&30.49&79.53&28.66\\
        &$\checkmark$&$\checkmark$&\textbf{84.80}&\textbf{22.73}&\textbf{84.74}&\textbf{23.43}\\
        \hline
    \end{tabular}
    }
    \vspace{-2pt}
    \caption{Ablation of the pretrain weight and backbones. `CLIP' indicates whether the image encoder uses CLIP based pretrain weight.}
    \label{table:ab2}
\end{table}


==> table/ablation3.tex <==

\begin{table}[!t]
    \centering
    \renewcommand\arraystretch{1.2}
    \resizebox{0.95\columnwidth}{!}{
    \begin{tabular}{c|cc|cc}
        \hline
        %\multicolumn{4}{|c|}{GCD-AVG}\\
        %\hline
        \multirow{2}*{Method} & \multicolumn{2}{c|}{Celeb-DF}&
        \multicolumn{2}{c}{DFDC-P}  \\
        \cline{2-5}
        % \cmidrule{2-5}
        & AUC& EER &AUC& EER \\
        \hline
        Coarse-Only&80.79&25.16&81.79&26.13\\
        % Fine-Only&64.29&29.29&65.99&38.13\\
        Fine-Pretrain&81.29&25.49&82.64&25.76\\
        Fine-and-Fine&82.19&24.43&82.95&25.53\\
        Coarse-and-Fine&\textbf{84.80}&\textbf{22.73}&\textbf{84.74}&\textbf{23.43}\\
        \hline
    \end{tabular}
    }
    \vspace{-2pt}
    \caption{Ablation of the different training strategy.}
    \label{table:ab3}
\end{table}


==> table/ablation4.tex <==

\begin{table}[!t]
    \centering
    \renewcommand\arraystretch{1.1}
    \resizebox{0.9\columnwidth}{!}{
    \begin{tabular}{c|cc|cc}
        \hline
        %\multicolumn{4}{|c|}{GCD-AVG}\\
        %\hline
        \multirow{2}*{Method} & \multicolumn{2}{c|}{Celeb-DF}&
        \multicolumn{2}{c}{DFDC-P}  \\
        \cline{2-5}
        % \cmidrule{2-5}
        & AUC& EER &AUC& EER \\
        \hline
        % Prompt1&77.21&29.55&77.39&30.36\\
        Prompt 1&82.17&25.18&79.19&26.13\\
        Prompt 2&80.60&26.78&82.04&26.26\\
        Prompt 3&83.32&24.40&83.09&24.90\\
        Prompt 4&\textbf{84.80}&\textbf{22.73}&\textbf{84.74}&\textbf{23.43}\\
        \hline
    \end{tabular}
    }
    \vspace{-2pt}
    \caption{Ablation of different coarse-grained prompts.}
    \label{table:ab4}
\end{table}


==> table/ablation_text.tex <==
% \begin{table}[!h]
%    \centering
%    \renewcommand\arraystretch{1.2}
%    \resizebox{1.0\columnwidth}{!}{
%    \begin{tabular}{c|c|c|c|c}
%        \hline
       
%         \multirow{2}*{Method} &\multicolumn{2}{c|}{Celeb-DF}&\multicolumn{2}{c}{DFDC-P}\\
%        \cline{2-5}

%        & AUC &EER& AUC &EER\\
%        \hline
%        Region(MC=4)&79.73&29.24&78.59&29.07\\
%        Region(MASK)&77.70&29.56&78.51&29.59\\
%        Region(Text)&\textbf{82.26}&\textbf{25.58}&\textbf{82.37}&\textbf{24.35}\\
%        \hline
%        Type(MC=31)&78.45&29.95&78.17&29.92\\
%        Type(Text)&\textbf{81.04}&\textbf{26.73}&\textbf{82.09}&\textbf{24.91}\\
%        \hline
%        Region+Type(MC=101)&77.18&30.47&77.54&31.03\\
%        Region+Type(Text)&\textbf{84.80}&\textbf{22.73}&\textbf{84.74}&\textbf{23.43}\\

%        \hline
%    \end{tabular}
%    }
%    \vspace{-8pt}
%    % \caption{Comparisons between Text and MC.}
%    \caption{Ablation study on text information and granularity of the fine-grained label. MC is represented as multiple classifiers. MASK means use mask as additional supervisory signal.}
%    \label{table:ablation}
% \end{table}


\begin{table}[!t]
   \centering
   \renewcommand\arraystretch{1.2}
   \resizebox{1.0\columnwidth}{!}{
   \begin{tabular}{c|c|c|c|c|c}
       \hline
       
        \multirow{2}*{Siginal}&\multirow{2}*{Method} &\multicolumn{2}{c|}{Celeb-DF}&\multicolumn{2}{c}{DFDC-P}\\
       \cline{3-6}

       && AUC &EER& AUC &EER\\
       \hline
       \multirow{1}*{Mask}&Decoder&77.70&29.56&78.51&29.59\\
       % &Decoder+PFIG&78.31&28.10&79.52&28.66\\
       \hline
       \multirow{3}*{Digital}&Region(MC=4)&79.73&29.24&78.59&29.07\\
       &Type(MC=31)&78.45&29.95&78.17&29.92\\
       &Region+Type(MC=101)&77.18&30.47&77.54&31.03\\
       \hline
       
       \multirow{3}*{Text}&Region&\textbf{82.26}&\textbf{25.58}&\textbf{82.37}&\textbf{24.35}\\
       &Type&\textbf{81.04}&\textbf{26.73}&\textbf{82.09}&\textbf{24.91}\\
       &Region+Type&\textbf{84.80}&\textbf{22.73}&\textbf{84.74}&\textbf{23.43}\\

       \hline
   \end{tabular}
   }
   % \vspace{-8pt}
   % \caption{Comparisons between Text and MC.}
   \caption{Ablation study on different supervisory signals. MC is represented as multiple classifiers.}
   \label{table:ablation}
\end{table}

==> table/tab1.tex <==

\begin{table*}[!h]
    \renewcommand\arraystretch{1.1}
    \centering
    \resizebox{0.95\textwidth}{!}{
    \begin{tabular}{l|cc|cccccccc}
    % \begin{tabular}{|ccccccccccc|}
    \hline
    \multirow{2}*{Method} & \multicolumn{2}{c|}{\textit{FF++}}&\multicolumn{2}{c}{DFD} & \multicolumn{2}{c}{DFDC-P} & \multicolumn{2}{c}{Wild Deepfake} &\multicolumn{2}{c}{Celeb-DF}\\
    % \cline{2-11}
    \cmidrule{2-3}
    \cmidrule{3-11}

    

    & AUC& EER &AUC& EER& AUC& EER& AUC& EER& AUC& EER\\
    \hline
    Xception~\cite{chollet2017xception}& 99.09&3.77 &87.86& 21.04& 69.80& 35.41&66.17 &40.14 & 65.27& 38.77\\
    % \hline
    EN-b4~\cite{tan2019efficientnet}   &99.22 &3.36& 87.37      & 21.99      & 70.12       & 34.54      & 61.04           & 45.34           & 68.52         & 35.61        \\
    % \hline
    Face X-ray~\cite{tan2019efficientnet}& 87.40&-& 85.60&-& 70.00&      -      &       -          &         -        & 74.20          &       -       \\
    % \hline
    % MLDG          &98.99 &3.46    & 88.14      & 21.34      & 71.86       & 34.44      & 64.12           & 43.27           & 74.56         & 30.81        \\
    % \hline
    
    % \hline
    F3-Net~\cite{qian2020thinking}          & 98.10& 3.58 & 86.10     & 26.17       &     72.88       &      33.38      & 67.71          &      40.17           & 71.21        &     34.03         \\
    MAT~\cite{zhao2021multi} & 99.27&3.35& 87.58      & 21.73      & 67.34       & 38.31      & 70.15           & 36.53           & 70.65         & 35.83        \\
    % \hline
    GFF~\cite{luo2021generalizing}             & 98.36& 3.85 & 85.51      & 25.64      & 71.58       & 34.77      & 66.51           & 41.52            & 75.31         & 32.48        \\
    % \hline
    LTW~\cite{sun2021domain}            & 99.17& 3.32  & 88.56      & 20.57      & 74.58       & 33.81      & 67.12           & 39.22           & 77.14         & 29.34         \\
    
    % \hline
    LRL~\cite{chen2021local}    & \textbf{99.46}&\textbf{3.01}& 89.24      & 20.32      & 76.53       & 32.41      & 68.76           & 37.50              & 78.26         & 29.67        \\
    
    DCL~\cite{sun2021dual}              & 99.30&3.26& 91.66      & 16.63      & 76.71       & 31.97      & 71.14         & 36.17           & 82.30       & 26.53   \\
    PCL+I2G~\cite{zhao2021learning}& 99.11&-& -      & -      & -       & -      & -         & -           & 81.80       & -   \\
    SBI~\cite{shiohara2022detecting}    & 88.33&20.47&88.13&17.25&76.53&30.22&68.22&38.11&80.76&26.97 \\
    UIA-ViT~\cite{zhuang2022uia} &-&-&94.68&-&75.80&-&-&-&82.41&- \\
    RECCE~\cite{cao2022end} &99.32&3.38&89.91&19.95&75.88&32.41&67.93&39.82&70.50&35.34 \\
    UCF~\cite{yan2023ucf} &97.05&-&80.74&-&75.94&-&-&-&75.27&- \\

    % UIA-ViT   & 99.33&-&94.68&-&75.80&-&-&-&82.41&- \\
    \hline

    Ours              & 99.23&3.12& \textbf{94.79}      & \textbf{15.31}      & \textbf{84.74}       & \textbf{23.43}      & \textbf{83.55}           & \textbf{24.40}           & \textbf{84.80}          & \textbf{22.73}       \\

    % Ours+Enhance              & 99.10&3.23& \textbf{95.05}      & \textbf{15.22}      & \textbf{85.22}       & \textbf{22.94}      & \underline{81.94}           & \underline{27.64}           & \textbf{85.22}          & \textbf{22.54}       \\

    
    \hline

    \end{tabular}
    }
    \caption{\textbf{Frame-level} cross-database evaluation from FF++(HQ) to DFD, DFDC-P, Wild Deepfake and Celeb-DF in terms of AUC and EER. The FF++ belongs to the intra-domain results while others represent the unseen-domain.
    }
    \label{table:1}
    \end{table*}


==> table/tab2_c40.tex <==

% \begin{table}[t!]
    
%     \renewcommand\arraystretch{1.4}
%     \centering
%     \resizebox{\columnwidth}{!}{
%     \begin{tabular}{ccc}
%         \hline
%         Method&FF++&Celeb-DF\\
%         \hline
%         Two-stream \cite{zhou2017two}&70.10&53.80\\
%         Meso-4\cite{afchar2018mesonet}&84.70&54.80\\
%         Mesoinception4\cite{afchar2018mesonet}&83.00&53.60\\
%         FWA\cite{li2018exposing}&80.10&56.90\\
%         DSP-FWA\cite{li2018exposing}&93.00&	64.60\\
%         Xception\cite{rossler2019faceforensics++}&95.50&65.50\\
%         Multi-task\cite{nguyen2019multi}&76.30&54.30\\
%         % Capeule\cite{nguyen2019use}&96.60&57.50\\
%         SMIL\cite{li2020sharp}&96.80&56.30\\
%         Two Branch\cite{masi2020two}&93.18&	73.41\\
%         EN-b4\cite{dolhansky2020deepfake}&96.39	&71.10\\
%         MAT\cite{zhao2021multi}&96.41&72.50	\\
%         GFF\cite{luo2021generalizing}&95.73&74.12\\
%         SPSL\cite{liu2021spatial}&96.91&	76.88\\
%         \hline
%         Ours&\textbf{96.97}&\textbf{81.00}\\
%         \hline
%     \end{tabular}
%     }
%      \vspace{-2pt}
%     \caption{Cross-dataset evaluation from FF++(LQ) to deepfake class of FF++ and Celeb-DF in terms of AUC. Some results
%     are from~\cite{masi2020two}, and the bold results are the best.}
%     \label{table:2}
% \end{table}

% \begin{table}[t!]
    
%     \renewcommand\arraystretch{1.2}
%     \centering
%     \resizebox{\columnwidth}{!}{
%     \begin{tabular}{c|c}
%         \hline
%         Method&Celeb-DF(AUC)\\
%         \hline
%         Two-stream \cite{zhou2017two}&53.80\\
%         Meso-4\cite{afchar2018mesonet}&54.80\\
%         Mesoinception4\cite{afchar2018mesonet}&53.60\\
%         FWA\cite{li2018exposing}&56.90\\
%         Xception\cite{rossler2019faceforensics++}&65.50\\
%         Multi-task\cite{nguyen2019multi}&54.30\\
%         % Capeule\cite{nguyen2019use}&57.50\\
%         DSP-FWA\cite{li2018exposing}&	64.60\\
%         SMIL\cite{li2020sharp}&56.30\\
%         Two Branch\cite{masi2020two}&	73.41\\
%         EN-b4\cite{dolhansky2020deepfake}&71.10\\
%         MAT\cite{zhao2021multi}&72.50	\\
%         F3-Net\cite{qian2020thinking}&65.17 \\
%         SPSL\cite{liu2021spatial}&	76.88\\
%         \hline
%         Ours&\textbf{81.00}\\
%         \hline
%     \end{tabular}
%     }
%      \vspace{-2pt}
%     \caption{Low quality image }
%     \label{table:2}
% \end{table}

\begin{table}[t!]
    
    \renewcommand\arraystretch{1.1}
    \centering.
    \resizebox{0.9\columnwidth}{!}{
    \begin{tabular}{c|cc}
        \hline
        Method&\quad   FF++ \quad  \quad&Celeb-DF\quad\\
        \hline
        % Two-stream &70.10&53.80\\
        Meso-4&84.70&54.80\\
        Mesoinception4&83.00&53.60\\
        FWA&80.10&56.90\\
        % DSP-FWA&93.00&	64.60\\
        Xception&95.50&65.50\\
        Multi-task&76.30&54.30\\
        % Capeule\cite{nguyen2019use}&96.60&57.50\\
        SMIL&96.80&56.30\\
        Two Branch&93.18&	73.41\\
        EN-b4&96.39	&71.10\\
        Multi-Attention&96.41&72.50	\\
        GFF&95.73&74.12\\
        SPSL&96.91&	76.88\\
        \hline
        Ours&\textbf{96.97}&\textbf{81.00}\\
        \hline
    \end{tabular}
    }
     
    \caption{Cross-dataset evaluation from FF++(LQ) to deepfake class of FF++ and Celeb-DF in terms of AUC.}
    
    \label{table:2}
\end{table}


==> table/tab3.tex <==
\begin{table*}[!t]
    \centering
    \renewcommand\arraystretch{1.1}
    \resizebox{0.95\textwidth}{!}{
        \scalebox{1}{
    \begin{tabular}{c|cc|cc|cc|cc}
        \hline
        \multirow{2}*{Method}& \multicolumn{2}{|l|}{GID-DF (HQ)} & \multicolumn{2}{l|}{GID-DF (LQ)} & \multicolumn{2}{l|}{GID-F2F (HQ)} & \multicolumn{2}{l}{GID-F2F (LQ)} \\
        \cline{2-9}
    & ACC            & AUC           & ACC            & AUC           & ACC            & AUC            & ACC            & AUC            \\
    \hline
    EN-B4         & 82.40           & 91.11         & 67.60           & 75.30          & 63.32          & 80.1           & 61.41           & 67.40           \\
    % \hline
    % Focalloss        & 81.33          & 90.31          & 67.47           & 74.95         & 60.80           & 79.80           & 61.00             & 67.21           \\
    % \hline
    % ForensicTransfer & 72.01          & -             & 68.20           & -             & 64.50           & -              & 55.00             & -              \\
    % \hline
    % Multi-task       & 70.30           & -             & 66.76           & -             & 58.74           & -              & 56.50           & -              \\
    % \hline
    % MLDG             & 84.21          & 91.82          & 67.15          & 73.12            & 63.46           & 77.10           & 58.12          & 61.70           \\
    % \hline
    LTW              & 85.60           & 92.70          & 69.15          & 75.60          & 65.60           & 80.20           & 65.70           & 72.40           \\

    DCL             & 87.70           & 94.9         & 75.90          & 83.82         & 68.40          & 82.93          & 67.85          & 75.07    \\
    
    Ours             & \textbf{92.47}           & \textbf{97.42}         & \textbf{82.14}          & \textbf{90.72}         & \textbf{69.12}          & \textbf{84.27}          & \textbf{71.94}          & \textbf{78.60}    \\
    \hline     
    UIA-ViT*             & 90.40           & 96.70         &  -         &     -     & 86.40          & 94.20     & -          & -    \\
        
    Ours*             & \textbf{94.22}           & \textbf{97.42}         & \textbf{85.33}          & \textbf{91.34}         & \textbf{87.93}          & \textbf{96.33}          & \textbf{73.22}          & \textbf{81.25}    \\
    \hline     

    \end{tabular}
    }
    }
    \caption{Performance on multi-source manipulation evaluation, the protocols and results are from \cite{sun2021domain}. GID-DF means traning on the other three manipulated methods of FF++ and test on deepfakes class. The same for the others.}
    \label{table:4}
    \end{table*}

% \begin{table*}[h!]
%     \resizebox{\textwidth}{!}{
%     \begin{tabular}{|l|l|l|l|l|l|l|l|l|}
%         \hline
%         \multirow{2}*{Method}& \multicolumn{2}{|l|}{GID-DF C23} & \multicolumn{2}{|l|}{GID-DF C40} & \multicolumn{2}{|l|}{GID-F2F C23} & \multicolumn{2}{|l|}{GID-F2F C40} \\
%         \cline{2-9}
%     & ACC            & AUC           & ACC            & AUC           & ACC            & AUC            & ACC            & AUC            \\
%     \hline
%     E-B0         & 82.4           & 91.11         & 67.6           & 75.3          & 63.32          & 80.1           & 61.4           & 67.4           \\
%     \hline
%     Focal        & 81.33          & 90.3          & 67.4           & 74.95         & 60.8           & 79.8           & 61             & 67.2           \\
%     \hline
%     FT & 72.01          & -             & 68.2           & -             & 64.5           & -              & 55             & -              \\
%     \hline
%     MT       & 70.3           & -             & 66.7           & -             & 58.7           & -              & 56.5           & -              \\
%     \hline
%     MLDG             & 84.21          & 91.8          & 67.15          & 73            & 63.4           & 77.1           & 58.12          & 61.7           \\
%     \hline
%     LTW              & 85.6           & 92.7          & 69.15          & 75.6          & 65.6           & 80.2           & 65.7           & 72.4           \\
%     \hline
%     ours             & 87.7           & 94.9         & 75.9          & 83.8         & 68.4          & 82.9          & 67.8          & 75.0    \\
%     \hline     
%     \end{tabular}
%     }
%     \caption{}
%     \label{table:4}

%     \end{table*}
